Thresholds for Reconstruction of Random Hypergraphs From Graph Projections

The graph projection of a hypergraph is a simple graph with the same vertex set and with an edge between each pair of vertices that appear in a hyperedge. We consider the problem of reconstructing a random $d$-uniform hypergraph from its projection. Feasibility of this task depends on $d$ and the density of hyperedges in the random hypergraph. For $d=3$ we precisely determine the threshold, while for $d\geq 4$ we give bounds. All of our feasibility results are obtained by exhibiting an efficient algorithm for reconstructing the original hypergraph, while infeasibility is information-theoretic. Our results also apply to mildly inhomogeneous random hypergrahps, including hypergraph stochastic block models (HSBM). A consequence of our results is an optimal HSBM recovery algorithm, improving on a result of Guadio and Joshi in 2023.

==> 2-connectivity-fig.tex <==
\begin{figure}
\centering
\begin{minipage}{.45\textwidth}

\centering
   % \resizebox{0.7\textwidth}{!}{
\begin{tikzpicture}[every node/.style={fill,circle,inner sep=1.5pt},yscale=0.9,xscale=0.8]

  % Define the coordinates for the shared vertices of orange triangles
  \coordinate (P1) at (0,0);
  \coordinate (P2) at (2,0);
  \coordinate (P3) at (1,1.732); % height of equilateral triangle
  \coordinate (P4) at (3,1.732);

  % Draw the orange triangles
  \filldraw[orange, fill=orange!20] (P1) -- (P2) -- (P3) -- cycle; % 1st triangle
  \filldraw[orange, fill=orange!20] (P2) -- (P3) -- (P4) -- cycle; % 2nd triangle
  \coordinate (P5) at (4,0); % Shift for the 3rd triangle
  \filldraw[orange, fill=orange!20] (P2) -- (P4) -- (P5) -- cycle; % 3rd triangle
  \coordinate (P6) at (5,1.732); % Height for the 4th triangle
  \filldraw[orange, fill=orange!20] (P4) -- (P5) -- (P6) -- cycle; % 4th triangle
  \coordinate (P7) at (1,-1.732);
  \filldraw[orange, fill=orange!20] (P1) -- (P2) --(P7) -- cycle;

  % Define the coordinates for the red triangles
  \coordinate (R1) at (5,-1.732);
  \coordinate (R2) at (6,0); 
  \coordinate (R3) at (7,-1.732);

  % Draw the red triangles
  \filldraw[red, fill=red!20] (P5) -- (R1) -- (R2) -- cycle; % 1st red triangle
  \filldraw[red, fill=red!20] (R2) -- (R1) -- (R3) -- cycle; % 2nd red triangle

  % The 3rd red triangle
  \coordinate (R4) at (8,0);
  \filldraw[red, fill=red!20] (R2) -- (R3) -- (R4) -- cycle;

  % Draw the 4-clique to the right
  \coordinate (C1) at (8,0); % Shared with 3rd red triangle
  \coordinate (C2) at (9,1);
  \coordinate (C3) at (9,-1);
  \coordinate (C4) at (10,0);
  \filldraw[blue, fill=blue!20] (R4) -- (C1) -- (C2) -- (C4) -- (C3) -- (C1); % Edges of 4-clique
  \draw[blue] (C2) -- (C3); % Diagonal of 4-clique
  \draw[blue] (C4) -- (C1); % Connect 3rd red triangle to 4-clique

  % Draw vertices of 4-clique
  % \foreach \i in {1,...,4}{
  %   \fill (C\i) circle [radius=2pt];
  % }
  % \fill (P1) circle [radius=2pt];
  % \fill (P2) circle [radius=2pt];
  % \fill (P3) circle [radius=2pt];
  % \fill (P4) circle [radius=2pt];
  % \fill (P5) circle [radius=2pt];
  % \fill (P6) circle [radius=2pt];
  % \fill (R1) circle [radius=2pt];
  % \fill (R2) circle [radius=2pt];
  % \fill (R3) circle [radius=2pt];
  % \fill (R4) circle [radius=2pt];
  % \fill (R5) circle [radius=2pt];
  
\end{tikzpicture}
         \caption{An example of hypergraph $H$. Triangles filled with colors represent hyperedges in $\hG$. Two hyperedges are 2-connected if they share two nodes. Different 2-connected components are marked in different colors. }
\label{fig:2-connectivity-H}
% \vspace{12mm}
\end{minipage}%
\hfill
\begin{minipage}{.45\textwidth}
\centering
   % \resizebox{0.7\textwidth}{!}{
\begin{tikzpicture}[,yscale=0.9,xscale=0.8]
  % Nodes
    % Define the coordinates for the shared vertices of orange triangles
  \coordinate (P1) at (0,0);
  \coordinate (P2) at (2,0);
  \coordinate (P3) at (1,1.732); % height of equilateral triangle
  \coordinate (P4) at (3,1.732);
  \coordinate (P5) at (4,0);
  \coordinate (P6) at (5,1.732);
  \coordinate (P7) at (1,-1.732);

    % Define the coordinates for the red triangles
  \coordinate (R1) at (5,-1.732);
  \coordinate (R2) at (6,0); 
  \coordinate (R3) at (7,-1.732);

    % Draw the 4-clique to the right
  \coordinate (C1) at (8,0); % Shared with 3rd red triangle
  \coordinate (C2) at (9,1);
  \coordinate (C3) at (9,-1);
  \coordinate (C4) at (10,0);
  \coordinate (C5) at (9,0);

  \node (b1) at (barycentric cs:P1=1,P2=1,P3=1) [circle, fill=orange, inner sep=1.5pt] {};
  \node (b2) at (barycentric cs:P2=1,P3=1,P4=1) [circle, fill=orange, inner sep=1.5pt] {};
  \node (b3) at (barycentric cs:P2=1,P4=1,P5=1) [circle, fill=orange, inner sep=1.5pt] {};
  \node (b4) at (barycentric cs:P4=1,P5=1,P6=1) [circle, fill=orange, inner sep=1.5pt] {};
  \node (b5) at (barycentric cs:P1=1,P2=1,P7=1) [circle, fill=orange, inner sep=1.5pt] {};

  % Draw lines between adjacent orange barycenters
  \draw[orange] (b1) -- (b2);
  \draw[orange] (b2) -- (b3);
  \draw[orange] (b3) -- (b4);
  \draw[orange] (b1) -- (b5);

  \node (br1) at (barycentric cs:P5=1,R1=1,R2=1) [circle, fill=red, inner sep=1.5pt] {};
  \node (br2) at (barycentric cs:R2=1,R1=1,R3=1) [circle, fill=red, inner sep=1.5pt] {};
  \node (br3) at (barycentric cs:R2=1,R3=1,C1=1) [circle, fill=red, inner sep=1.5pt] {};
  \draw[red] (br1) -- (br2) -- (br3);

    \node (bc1) at (barycentric cs:C1=1,C2=1,C5=1) [circle, fill=blue, inner sep=1.5pt] {};
  \node (bc2) at (barycentric cs:C2=1,C4=1,C5=1) [circle, fill=blue, inner sep=1.5pt] {};
  \node (bc3) at (barycentric cs:C3=1,C4=1,C5=1) [circle, fill=blue, inner sep=1.5pt] {};
  \node (bc4) at (barycentric cs:C3=1,C1=1,C5=1) [circle, fill=blue, inner sep=1.5pt] {};
  \draw[blue] (bc1) -- (bc2) -- (bc3) -- (bc4) -- (bc1);
\end{tikzpicture}
         \caption{The corresponding graph $\cG_H$. Each node in $\cG_H$ corresponds to a hyperedge in $H$. Two nodes are connected if their corresponding hyperedges share two nodes.}
         % \label{fig:three sin x}
     % \end{subfigure}
% \caption{An example of  2-connectivity and 2-connected components when $d=3$.}
\label{fig:2-connectivity-G}
\end{minipage}
\end{figure}

==> AuthorFeedback/macros-response.tex <==
\usepackage[utf8]{inputenc}
\usepackage{amsmath}
\usepackage{amssymb,amsfonts}
\usepackage{mathrsfs}
\usepackage{algorithm}
% \usepackage{algorithmic}
\usepackage{xcolor}
\usepackage{tikz}
\usepackage{fullpage}
\usepackage{dsfont}
\usepackage{thmtools}
\usepackage{thm-restate}
\usepackage{enumitem}
\usepackage[noend]{algpseudocode}
\usepackage{subcaption}
\usepackage{graphicx}
\usetikzlibrary{shapes,arrows,backgrounds,fit,positioning,calc}

% \usepackage{authblk}

\usepackage{hyperref}
\usepackage{cleveref}
\usepackage{xcolor}
\hypersetup{
  colorlinks   = true, %Colours links instead of ugly boxes
  urlcolor     = blue, %Colour for external hyperlinks
  linkcolor    = blue, %Colour of internal links
  citecolor   = blue %Colour of citations
}

\usepackage{tikz}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{arrows,positioning}
%
%%SetFonts
\DeclareRobustCommand\shape{
 \lower5pt\hbox{
 \hskip-7pt
  \tikzset{circ/.style={circle, draw, fill=black, scale=.15}}
  \begin{tikzpicture}[semithick,scale=.3]
  \node (l1) at (0,.5) [circ]{};
%   \node (l2) at (1,.866) [circ]{};
  \node (l3) at (0.5,0.3) [circ]{};
    % \draw[-,color=white] (l1) to node [auto] {} (l2);
  \draw[-] (l1) to node [auto] {} (l3);
%   \draw[-] (l2) to node [auto] {} (l3);
    \end{tikzpicture}
  \hskip-8pt}
}
% \def\Vshape{
%   \draw[-,color=white] (l1) to node [auto] {} (l2);
%   \draw[-] (l1) to node [auto] {} (l3);
%   \draw[-] (l2) to node [auto] {} (l3);
% }

\newcommand{\bern}{\mathsf{Bern}}
\newcommand{\unif}{\mathsf{Unif}}



% \newtheorem{conjecture}{Conjecture}[]
% \newtheorem{theorem}{Theorem}[section]

\newtheorem{innercustomlem}{Lemma}
\newenvironment{mylem}[1]
  {\renewcommand\theinnercustomlem{#1}\innercustomlem}
  {\endinnercustomlem}

  \newtheorem{innercustomthm}{Theorem}
\newenvironment{mythm}[1]
  {\renewcommand\theinnercustomthm{#1}\innercustomthm}
  {\endinnercustomthm}

% \newtheorem{lemma}{Lemma}[section]
% \newtheorem{corollary}[lemma]{Corollary}
% \newtheorem{fact}{Fact}
% \theoremstyle{definition}
% \newtheorem{remark}{Remark}[]
% \newtheorem{definition}{Definition}
% \newtheorem{problem}{Problem}[]

%macros 
\newcommand{\var}{\mathsf{Var}}
\DeclareMathOperator*{\E}{{\rm I}\kern-0.18em{\rm E}}
% \newcommand{\E}{\,{\rm I}\kern-0.18em{\rm E}}
\renewcommand{\Pr}{\,{\rm I}\kern-0.18em{\rm P}}
\newcommand{\1}{\mathds{1}}
\newcommand{\ind}[1]{\1\{#1\}}
\newcommand{\poi}{\mathrm{Poisson}}
\newcommand{\bino}{\mathsf{Binomial}}
\newcommand{\multino}{\mathsf{Multinomial}}
\newcommand{\TV}{{d_\mathsf{TV}}}
\newcommand{\RES}{\mathsf{Res}}
\newcommand{\law}{\mathcal{L}}
\newcommand{\rgt}{\mathsf{RGT}}
\newcommand{\rig}{\mathsf{RIG}}
\newcommand{\G}{\mathsf{G}}
\newcommand{\disteq}{\stackrel{d}{=}}
\newcommand{\gd}{\mathsf{P_{GD}}}
\newcommand{\defeq}{\triangleq}
% {\stackrel{\text{def}}{=}}
\newcommand{\rg}{\mathsf{P_0}}
\newcommand{\prg}{\mathsf{P_1}}
\newcommand{\prgp}{\mathsf{P'_1}}
\newcommand{\rigp}{\mathsf{RIG_P}}
\newcommand{\rigpf}{\mathsf{RIG_{P4}}}
\newcommand{\inv}{^{-1}}

\newcommand{\spacedot}{\,\cdot\,}

\newcommand{\e}{\mathsf{e}}

\newcommand{\B}{\Big}
\renewcommand{\b}{\big}

\newcommand{\red}[1]{{\color{red}#1}}

\newcommand{\gb}[1]{{{\color{magenta}\texttt{[#1]}}}}
% \newcommand{\gb}[1]{}
\newcommand{\gbdone}[1]{{\color{blue}\texttt{[#1]}}}
\newcommand{\cg}[1]{{\color{green}\texttt{[#1]}}}
% \newcommand{\cg}[1]{}

\newcommand{\up}[1]{^{(#1)}}

\newcommand{\dotspace}{\,\cdot\,}

\newcommand{\fresh}[1]{\textcolor{blue}{#1}}

\newcommand{\muge}[1]{\mu^{\shape{}}_{#1}}
\newcommand{\mug}[1]{\mu_{#1}}

\newcommand{\IM}[2]{\Inf^M_{#1\rightarrow #2}}

\newcommand{\I}[2]{\Inf_{#1\rightarrow #2}}

\newcommand{\Inf}{\mathbf{I}}

\newcommand{\ER}{{Erd\H os-R\'enyi}}

\newcommand{\appeq}[1]{\stackrel{#1}{\approx }}

\newcommand{\aux}{X^{\mathsf{aux}}}

\newcommand{\enew}{E^{\mathsf{new}}}

\def\nbyp#1{\textcolor{red}{[{\bf YP:} #1]}}

\newcommand{\ERi}[1]{G_{#1}}

\newcommand{\RGTi}[1]{\rgt_{#1}}

\newcommand{\wed}[1][]{W_{#1}}

\newcommand{\bwed}[1][]{\bar{W}_{#1}}

\newcommand{\Twed}{\bar{T}}

\newcommand{\pdist}[2]{P_{(#1,#2)}}

%caligraphic


\newcommand{\cX}{\mathcal{X}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\bN}{\mathbb{N}}
\newcommand{\cN}{\mathbb{M}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cK}{\mathcal{K}}

\newcommand{\norm}[1]{\|#1\|}


\newcommand{\quadand}{\quad\text{and}\quad}

\newcommand{\ssbm}{\mathsf{G_B}}
\newcommand{\ssbmrgt}{\mathsf{RGT_B}}
\newcommand{\gps}{\mathsf{GPS}}
\newcommand{\easy}{\mathsf{easy}}
\newcommand{\hard}{\mathsf{hard}}
\newcommand{\impo}{\mathsf{impossible}}
\newcommand{\pd}{\mathsf{PD}}
\newcommand{\gl}{\mathsf{D}_{gl}}

\newcommand{\cov}{\mathsf{Cov}}


\newcommand{\Ot}{\tilde{O}}

\newcommand{\Tht}{\tilde{\Theta}}

\newcommand{\sn}{\sqrt{n}}


\newcommand{\ep}{1/r^2}
\newcommand{\mcover}{\mathcal{C}}
\newcommand{\pinc}{p_{inc}}
\newcommand{\cS}{\mathcal{S}}

\newcommand{\hG}{H}
\newcommand{\rhG}{\cH}
\newcommand{\hE}{\cE}
\newcommand{\he}{h}
\newcommand{\pG}{{G_p}}
\newcommand{\pE}{E_p}
\newcommand{\cliG}{{\rhG_c}}
\newcommand{\cliE}{\cE_c}
\newcommand{\proj}{\mathrm{Proj}}
\newcommand{\Ih}{{X}}
\newcommand{\Ip}{{Y}}
\newcommand{\Ic}{{Z}}
\newcommand{\prim}{{\mathrm{Proj}^{-1}}}
\newcommand{\cli}{\mathrm{Cli}}
\newcommand{\nei}[1]{N_{#1}}
\newcommand{\aG}{G_{a,d}}
\newcommand{\cdel}[1]{\delta^*_{#1}}
\newcommand{\cliA}{\cA_c}
\newcommand{\naH}{{H_f}}
\newcommand{\aut}{\mathrm{aut}}
\newcommand{\chG}[1]{K_n^{(#1)}}
\newcommand{\bG}{\hG_b}

\newcommand{\hsbm}{\mathrm{HSBM}}
\newcommand{\grow}{\mathrm{Grow}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}


==> Connectevity.tex <==

\section{MAP is Efficient for Sparse Hypergraphs}


% This allows us to output a minimum pre-image

% \begin{lemma}\label{lem:component-constant-size}
%     For any $\delta<\frac{d-1}{d+1}$, any 2-connected component of $\cliG$ has size at most $\frac{2}{\frac{d-1}{d+1}-\delta}=O_n(1)$ with high probability.
% \end{lemma}
% \begin{proof}
% For any $\he_1\in \binom{[n]}{d}$,
% let $C(\he_1)$ be the 2-connected component of $\cliG$ that contains $\he_1$ if $\he_1\in\hE_\rhG$ and $\emptyset$ otherwise. Let us control the probability that a 2-connected component grows from size $t-1$ to size $t$.
% % , we let $C(\he_1)=\emptyset$ if $\he_1\not \in \cliG$. For any $t\in\mathbb{Z}^+$,
% \[
% \begin{split}
%     &\Pr\b(|C(\he_1)|\ge t\b| |C(\he_1)|\ge t-1\b)\\
%     &=\Pr\b(\nei{\cliG}(\{\he_1,\cdots, \he_{t-1}\})\ne\emptyset \b| \exists h_1,\cdots, h_{t-1}\in\cliG \text{ s.t. }\{\he_1,\cdots, \he_{t-1}\}\text{ is 2-connected}\b)\\
%     &= \Pr\b(\nei{\cliG}(\{\he_1,\cdots, \he_{t-1}\})\ne\emptyset \b| \exists \text{a minimal cover $\hE$ of } h_1,\cdots, h_{t-1}\in\binom{[n]}{d}\text{ s.t. }   \{\he_1,\cdots, \he_{t-1}\}\text{ is 2-connected}, \hE\subset \hE_\rhG\b)
% \end{split}
% \]
% For any $t=O_n(1)$, any minimal cover of $h_1,\cdots, h_{t-1}$ also has size $O_n(1)$. So by Lemma~\ref{lem:branching}, 
% \[
% \Pr\b(|C(\he_1)|\ge t\b| |C(\he_1)|\ge t-1\b)=O_n(n^{-(\frac{d-1}{d+1}-\delta)})\,.
% \]
% So we have
% \[
% \begin{split}
% &\Pr(|C(\he_1)|\ge k)\\
% &=\Pr(\he_1\in \hE_\rhG)\prod_{t=2}^k\Pr\b(|C(\he_1)|\ge t\b| |C(\he_1)|\ge t-1\b)\\
% &=O_n(n^{-d+1+\delta}\cdot n^{-(k-1)(\frac{d-1}{d+1}-\delta)})\,.
% \end{split}
% \]
% Union bound over all $\he_1\in\binom{[n]}{d}$ and set $k=1+\frac{2}{\frac{d-1}{d+1}-\delta}$, we get 
% \[
% \Pr\B(\exists\he_1\in\binom{[n]}{d} , |C(\he_1)|\ge k\B) \le \binom{n}{d}O_n(n^{-d+1+\delta-(k-1)(\frac{d-1}{d+1}-\delta)}) = O_n(n^{\delta-1})=o_n(1)\,.
% \]
% This means any 2-connected component of $\cliG$ has size at most $k-1=\frac{2}{\frac{d-1}{d+1}-\delta}$ with probability $1-o_n(1)$.
% % Let  $\he_i$ to be a random hyperedge in $\nei{\cliG}(\{\he_0,\he_1,\cdots, \he_{i-1}$
% % We have
% % \[
% % |C(\he_0)|\ge t\Leftrightarrow \exists \he_1\in \nei{\cliG}(\he_0), \exists \he_2\in \nei{\cliG}(\{\he_0,\he_1\})\cdots, \exists \he_t\in \nei{\cliG}(\{\he_0,\he_1,\cdots, \he_{t-1}\})
% % \]
% % So 
% % \[
% % \Pr(|C(\he_0)|\ge t) = \prod_{i=1}^t \Pr(\exists \he_t\in \nei{\cliG}(\{\he_0,\he_1,\cdots, \he_{t-1}\}) | )
% % \]
% \end{proof}

\nbyp{I don't understand this lemma. It seems that $Proj(\mathcal{E}_1)$ is missing, but also what is the role of $\mathcal{E}_0$?}
\cg{rewrite this part}
\begin{lemma}\label{lem:branching}
For any $\hE_1\subset \binom{[n]}{d}$ with $|\hE_1|=O_n(1)$,
\[
    \Pr\b(\nei{\cliG}(\cli(\hE_1))\ne \emptyset | \hE_1\subset \hE_{\rhG}\b) =
    \begin{cases}
        O_n(n^{-(\frac{d-1}{d+1}-\delta)}) &\text{if }\delta<\frac{d-1}{d+1}\\
        1-\Omega_n(1) &\text{if }\delta=\frac{d-1}{d+1}
    \end{cases}
    \,.
\]


\end{lemma}


% We can show that the above bound is tight, \cg{delete}
% \begin{lemma}\label{lem:branching-tight}
%     When $\delta>\frac{d-1}{d+1}$, there exists $\hE_1\subset \binom{[n]}{d}$ such that 
%     \[
%     \Pr\b(\nei{\cliG}(\cli(\hE_1))\ne \emptyset | \hE_1\subset \hE_{\rhG}\b) = 1-o_n(1)\,.
%     \]
% \end{lemma}
\begin{proof}
% Note that the event $\nei{\cliG}(\cli(\hE_1))\ne \emptyset$ is monotonically increasing in all hyperedges, by Harris inequality, we have 
% \[
% \Pr\b(\nei{\cliG}(\cli(\hE_1))\ne \emptyset | \hE_1\subset \hE_{\rhG}, \hE_0\cap \hE_{\rhG}=\emptyset\b) \le \Pr\b(\nei{\cliG}(\cli(\hE_1))\ne \emptyset | \hE_1\subset \hE_{\rhG}\b)\,.
% \]
% In other words, we can consider the case when $\hE_0$ is empty without loss of generality. 

\end{proof}





==> Preliminary.tex <==
% \section{Preliminaries}
% A \emph{random $d$-hypergraph} $\rhG(n,d,\delta)=([n],\hE_{\hG})$ \footnote{\cg{might be helpful to have separate notations for a set of hyperedges and a set of edges}} where every $d$-hyperedge is included in $\hE_{\rhG}$ with probability $p=\Theta(n^{-d+1+\delta})$.\footnote{Constant factors do not affect any result of the paper. The same result also holds with possibly different probabilities at different edges. The parametrization is made so that expected degree of a node is $\Theta(n^\delta)$.} 
% Let $\Ih_\he$ for any $\he\in \binom{[n]}{d}$ be the indicator that $\he\in \hE_{\rhG}$.







==> temporaryMacrosEtc/macros.tex <==
% \usepackage[utf8]{inputenc}
%\usepackage{amsmath}
%\usepackage{amssymb,amsfonts,amsthm}
%\usepackage{mathrsfs}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{xcolor}
\usepackage{tikz}
\usepackage{fullpage}
\usepackage{dsfont}
\usepackage{thmtools}
\usepackage{thm-restate}
\usepackage{enumitem}
% \usepackage[noend]{algpseudocode}
\usepackage{subcaption}
\usepackage{graphicx}
\usetikzlibrary{shapes,arrows,backgrounds,fit,positioning}

% \usepackage{authblk}

\usepackage{hyperref}
\usepackage{cleveref}
\usepackage{xcolor}
\hypersetup{
  colorlinks   = true, %Colours links instead of ugly boxes
  urlcolor     = blue, %Colour for external hyperlinks
  linkcolor    = blue, %Colour of internal links
  citecolor   = blue %Colour of citations
}

\usepackage{tikz}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{arrows,positioning}
%
%%SetFonts
\DeclareRobustCommand\shape{
 \lower5pt\hbox{
 \hskip-7pt
  \tikzset{circ/.style={circle, draw, fill=black, scale=.15}}
  \begin{tikzpicture}[semithick,scale=.3]
  \node (l1) at (0,.5) [circ]{};
%   \node (l2) at (1,.866) [circ]{};
  \node (l3) at (0.5,0.3) [circ]{};
    % \draw[-,color=white] (l1) to node [auto] {} (l2);
  \draw[-] (l1) to node [auto] {} (l3);
%   \draw[-] (l2) to node [auto] {} (l3);
    \end{tikzpicture}
  \hskip-8pt}
}
% \def\Vshape{
%   \draw[-,color=white] (l1) to node [auto] {} (l2);
%   \draw[-] (l1) to node [auto] {} (l3);
%   \draw[-] (l2) to node [auto] {} (l3);
% }

\newcommand{\bern}{\mathsf{Bern}}
\newcommand{\unif}{\mathsf{Unif}}



%\newtheorem{conjecture}{Conjecture}[]
%\newtheorem{theorem}{Theorem}[section]

\newtheorem{innercustomlem}{Lemma}
\newenvironment{mylem}[1]
  {\renewcommand\theinnercustomlem{#1}\innercustomlem}
  {\endinnercustomlem}

  \newtheorem{innercustomthm}{Theorem}
\newenvironment{mythm}[1]
  {\renewcommand\theinnercustomthm{#1}\innercustomthm}
  {\endinnercustomthm}

%\newtheorem{lemma}{Lemma}[section]
%\newtheorem{corollary}[lemma]{Corollary}
%\newtheorem{fact}{Fact}
%\theoremstyle{definition}
%\newtheorem{remark}{Remark}[]
%\newtheorem{definition}{Definition}
%\newtheorem{problem}{Problem}[]
%
%macros 
\newcommand{\var}{\mathsf{Var}}
\DeclareMathOperator*{\E}{{\rm I}\kern-0.18em{\rm E}}
% \newcommand{\E}{\,{\rm I}\kern-0.18em{\rm E}}
\renewcommand{\Pr}{\,{\rm I}\kern-0.18em{\rm P}}
\newcommand{\1}{\mathds{1}}
\newcommand{\ind}[1]{\1\{#1\}}
\newcommand{\poi}{\mathrm{Poisson}}
\newcommand{\bino}{\mathsf{Binomial}}
\newcommand{\multino}{\mathsf{Multinomial}}
\newcommand{\TV}{{d_\mathsf{TV}}}
\newcommand{\RES}{\mathsf{Res}}
\newcommand{\law}{\mathcal{L}}
\newcommand{\rgt}{\mathsf{RGT}}
\newcommand{\rig}{\mathsf{RIG}}
\newcommand{\G}{\mathsf{G}}
\newcommand{\disteq}{\stackrel{d}{=}}
\newcommand{\gd}{\mathsf{P_{GD}}}
\newcommand{\defeq}{\triangleq}
% {\stackrel{\text{def}}{=}}
\newcommand{\rg}{\mathsf{P_0}}
\newcommand{\prg}{\mathsf{P_1}}
\newcommand{\prgp}{\mathsf{P'_1}}
\newcommand{\rigp}{\mathsf{RIG_P}}
\newcommand{\rigpf}{\mathsf{RIG_{P4}}}
\newcommand{\inv}{^{-1}}

\newcommand{\spacedot}{\,\cdot\,}

\newcommand{\e}{\mathsf{e}}

\newcommand{\B}{\Big}
\renewcommand{\b}{\big}

\newcommand{\red}[1]{{\color{red}#1}}

\newcommand{\gb}[1]{}
\newcommand{\gbdone}[1]{}
% \newcommand{\cg}[1]{{\color{green}\texttt{[#1]}}}
\newcommand{\cg}[1]{}

\newcommand{\up}[1]{^{(#1)}}

\newcommand{\dotspace}{\,\cdot\,}

\newcommand{\fresh}[1]{\textcolor{blue}{#1}}

\newcommand{\muge}[1]{\mu^{\shape{}}_{#1}}
\newcommand{\mug}[1]{\mu_{#1}}

\newcommand{\IM}[2]{\Inf^M_{#1\rightarrow #2}}

\newcommand{\I}[2]{\Inf_{#1\rightarrow #2}}

\newcommand{\Inf}{\mathbf{I}}

\newcommand{\ER}{{Erd\H{o}s-R\'enyi}}

\newcommand{\appeq}[1]{\stackrel{#1}{\approx }}

\newcommand{\aux}{X^{\mathsf{aux}}}

\newcommand{\enew}{E^{\mathsf{new}}}

\def\nbyp#1{\textcolor{red}{[{\bf YP:} #1]}}

\newcommand{\ERi}[1]{G_{#1}}

\newcommand{\RGTi}[1]{\rgt_{#1}}

\newcommand{\wed}[1][]{W_{#1}}

\newcommand{\bwed}[1][]{\bar{W}_{#1}}

\newcommand{\Twed}{\bar{T}}

\newcommand{\pdist}[2]{P_{(#1,#2)}}

%caligraphic

\newcommand{\cX}{\mathcal{X}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\bN}{\mathbb{N}}
\newcommand{\cN}{\mathbb{M}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cK}{\mathcal{K}}

\newcommand{\norm}[1]{\|#1\|}


\newcommand{\quadand}{\quad\text{and}\quad}

\newcommand{\ssbm}{\mathsf{G_B}}
\newcommand{\ssbmrgt}{\mathsf{RGT_B}}
\newcommand{\gps}{\mathsf{GPS}}
\newcommand{\easy}{\mathsf{easy}}
\newcommand{\hard}{\mathsf{hard}}
\newcommand{\impo}{\mathsf{impossible}}
\newcommand{\pd}{\mathsf{PD}}
\newcommand{\gl}{\mathsf{D}_{gl}}

\newcommand{\cov}{\mathsf{Cov}}


\newcommand{\Ot}{\tilde{O}}

\newcommand{\Tht}{\tilde{\Theta}}

\newcommand{\sn}{\sqrt{n}}


\newcommand{\ep}{1/r^2}
\newcommand{\mcover}{\mathcal{C}}
\newcommand{\pinc}{p_{inc}}
\newcommand{\cS}{\mathcal{S}}

\newcommand{\hG}{H}
\newcommand{\rhG}{\cH}
\newcommand{\hE}{\cE}
\newcommand{\he}{h}
\newcommand{\pG}{{G_p}}
\newcommand{\pE}{E_p}
\newcommand{\cliG}{{\rhG_c}}
\newcommand{\cliE}{\cE_c}
\newcommand{\proj}{\mathrm{Proj}}
\newcommand{\Ih}{{X}}
\newcommand{\Ip}{{Y}}
\newcommand{\Ic}{{Z}}
\newcommand{\prim}{{\mathrm{Proj}^{-1}}}
\newcommand{\cli}{\mathrm{Cli}}
\newcommand{\nei}[1]{N_{#1}}
\newcommand{\aG}{G_{a,d}}
\newcommand{\cdel}[1]{\delta^*_{#1}}
\newcommand{\cliA}{\cA_c}
\newcommand{\naH}{H}
\newcommand{\aut}{\mathrm{aut}}
\newcommand{\chG}[1]{K_n^{(#1)}}
\newcommand{\bG}{\hG_b}

\newcommand{\hsbm}{\mathrm{HSBM}}
\newcommand{\grow}{\mathrm{Grow}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}


==> temporaryMacrosEtc/macrosOLD.tex <==
\usepackage[utf8]{inputenc}
\usepackage{amsmath}
\usepackage{amssymb,amsfonts,amsthm}
\usepackage{mathrsfs}
\usepackage{algorithm}
% \usepackage{algorithmic}
\usepackage{xcolor}
\usepackage{tikz}
\usepackage{fullpage}
\usepackage{dsfont}
\usepackage{thmtools}
\usepackage{thm-restate}
\usepackage{enumitem}
\usepackage[noend]{algpseudocode}
\usepackage{subcaption}
\usepackage{graphicx}
\usetikzlibrary{shapes,arrows,backgrounds,fit,positioning}

% \usepackage{authblk}

\usepackage{hyperref}
\usepackage{cleveref}
\usepackage{xcolor}
\hypersetup{
  colorlinks   = true, %Colours links instead of ugly boxes
  urlcolor     = blue, %Colour for external hyperlinks
  linkcolor    = blue, %Colour of internal links
  citecolor   = blue %Colour of citations
}

\usepackage{tikz}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{arrows,positioning}
%
%%SetFonts
\DeclareRobustCommand\shape{
 \lower5pt\hbox{
 \hskip-7pt
  \tikzset{circ/.style={circle, draw, fill=black, scale=.15}}
  \begin{tikzpicture}[semithick,scale=.3]
  \node (l1) at (0,.5) [circ]{};
%   \node (l2) at (1,.866) [circ]{};
  \node (l3) at (0.5,0.3) [circ]{};
    % \draw[-,color=white] (l1) to node [auto] {} (l2);
  \draw[-] (l1) to node [auto] {} (l3);
%   \draw[-] (l2) to node [auto] {} (l3);
    \end{tikzpicture}
  \hskip-8pt}
}
% \def\Vshape{
%   \draw[-,color=white] (l1) to node [auto] {} (l2);
%   \draw[-] (l1) to node [auto] {} (l3);
%   \draw[-] (l2) to node [auto] {} (l3);
% }

\newcommand{\bern}{\mathsf{Bern}}
\newcommand{\unif}{\mathsf{Unif}}



% \newtheorem{conjecture}{Conjecture}[]
\newtheorem{theorem}{Theorem}[section]

\newtheorem{innercustomlem}{Lemma}
\newenvironment{mylem}[1]
  {\renewcommand\theinnercustomlem{#1}\innercustomlem}
  {\endinnercustomlem}

  \newtheorem{innercustomthm}{Theorem}
\newenvironment{mythm}[1]
  {\renewcommand\theinnercustomthm{#1}\innercustomthm}
  {\endinnercustomthm}

\newtheorem{lemma}{Lemma}[section]
\newtheorem{corollary}[lemma]{Corollary}
% \newtheorem{fact}{Fact}
% \theoremstyle{definition}
\newtheorem{remark}{Remark}[]
\newtheorem{definition}{Definition}
% \newtheorem{problem}{Problem}[]

%macros 
\newcommand{\var}{\mathsf{Var}}
\DeclareMathOperator*{\E}{{\rm I}\kern-0.18em{\rm E}}
% \newcommand{\E}{\,{\rm I}\kern-0.18em{\rm E}}
\renewcommand{\Pr}{\,{\rm I}\kern-0.18em{\rm P}}
\newcommand{\1}{\mathds{1}}
\newcommand{\ind}[1]{\1\{#1\}}
\newcommand{\poi}{\mathrm{Poisson}}
\newcommand{\bino}{\mathsf{Binomial}}
\newcommand{\multino}{\mathsf{Multinomial}}
\newcommand{\TV}{{d_\mathsf{TV}}}
\newcommand{\RES}{\mathsf{Res}}
\newcommand{\law}{\mathcal{L}}
\newcommand{\rgt}{\mathsf{RGT}}
\newcommand{\rig}{\mathsf{RIG}}
\newcommand{\G}{\mathsf{G}}
\newcommand{\disteq}{\stackrel{d}{=}}
\newcommand{\gd}{\mathsf{P_{GD}}}
\newcommand{\defeq}{\triangleq}
% {\stackrel{\text{def}}{=}}
\newcommand{\rg}{\mathsf{P_0}}
\newcommand{\prg}{\mathsf{P_1}}
\newcommand{\prgp}{\mathsf{P'_1}}
\newcommand{\rigp}{\mathsf{RIG_P}}
\newcommand{\rigpf}{\mathsf{RIG_{P4}}}
\newcommand{\inv}{^{-1}}

\newcommand{\spacedot}{\,\cdot\,}

\newcommand{\e}{\mathsf{e}}

\newcommand{\B}{\Big}
\renewcommand{\b}{\big}

\newcommand{\red}[1]{{\color{red}#1}}

% \newcommand{\gb}[1]{{{\color{magenta}\texttt{[#1]}}}}
\newcommand{\gb}[1]{}
\newcommand{\gbdone}[1]{{\color{blue}\texttt{[#1]}}}
% \newcommand{\cg}[1]{{\color{green}\texttt{[#1]}}}
\newcommand{\cg}[1]{}

\newcommand{\up}[1]{^{(#1)}}

\newcommand{\dotspace}{\,\cdot\,}

\newcommand{\fresh}[1]{\textcolor{blue}{#1}}

\newcommand{\muge}[1]{\mu^{\shape{}}_{#1}}
\newcommand{\mug}[1]{\mu_{#1}}

\newcommand{\IM}[2]{\Inf^M_{#1\rightarrow #2}}

\newcommand{\I}[2]{\Inf_{#1\rightarrow #2}}

\newcommand{\Inf}{\mathbf{I}}

\newcommand{\ER}{{Erd\H{o}s-R\'enyi}}

\newcommand{\appeq}[1]{\stackrel{#1}{\approx }}

\newcommand{\aux}{X^{\mathsf{aux}}}

\newcommand{\enew}{E^{\mathsf{new}}}

\def\nbyp#1{\textcolor{red}{[{\bf YP:} #1]}}

\newcommand{\ERi}[1]{G_{#1}}

\newcommand{\RGTi}[1]{\rgt_{#1}}

\newcommand{\wed}[1][]{W_{#1}}

\newcommand{\bwed}[1][]{\bar{W}_{#1}}

\newcommand{\Twed}{\bar{T}}

\newcommand{\pdist}[2]{P_{(#1,#2)}}

%caligraphic

\newcommand{\cX}{\mathcal{X}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\bN}{\mathbb{N}}
\newcommand{\cN}{\mathbb{M}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cK}{\mathcal{K}}

\newcommand{\norm}[1]{\|#1\|}


\newcommand{\quadand}{\quad\text{and}\quad}

\newcommand{\ssbm}{\mathsf{G_B}}
\newcommand{\ssbmrgt}{\mathsf{RGT_B}}
\newcommand{\gps}{\mathsf{GPS}}
\newcommand{\easy}{\mathsf{easy}}
\newcommand{\hard}{\mathsf{hard}}
\newcommand{\impo}{\mathsf{impossible}}
\newcommand{\pd}{\mathsf{PD}}
\newcommand{\gl}{\mathsf{D}_{gl}}

\newcommand{\cov}{\mathsf{Cov}}


\newcommand{\Ot}{\tilde{O}}

\newcommand{\Tht}{\tilde{\Theta}}

\newcommand{\sn}{\sqrt{n}}


\newcommand{\ep}{1/r^2}
\newcommand{\mcover}{\mathcal{C}}
\newcommand{\pinc}{p_{inc}}
\newcommand{\cS}{\mathcal{S}}

\newcommand{\hG}{H}
\newcommand{\rhG}{\cH}
\newcommand{\hE}{\cE}
\newcommand{\he}{h}
\newcommand{\pG}{{G_p}}
\newcommand{\pE}{E_p}
\newcommand{\cliG}{{\rhG_c}}
\newcommand{\cliE}{\cE_c}
\newcommand{\proj}{\mathrm{Proj}}
\newcommand{\Ih}{{X}}
\newcommand{\Ip}{{Y}}
\newcommand{\Ic}{{Z}}
\newcommand{\prim}{{\mathrm{Proj}^{-1}}}
\newcommand{\cli}{\mathrm{Cli}}
\newcommand{\nei}[1]{N_{#1}}
\newcommand{\aG}{G_{a,d}}
\newcommand{\cdel}[1]{\delta^*_{#1}}
\newcommand{\cliA}{\cA_c}
\newcommand{\naH}{H}
\newcommand{\aut}{\mathrm{aut}}
\newcommand{\chG}[1]{K_n^{(#1)}}
\newcommand{\bG}{\hG_b}

\newcommand{\hsbm}{\mathrm{HSBM}}
\newcommand{\grow}{\mathrm{Grow}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

